Solving String Constraints With Regex-Dependent Functions Through Transducers With Priorities And Variables

Regular expressions are a classical concept in formal language theory. Regular expressions in programming languages (RegEx) such as JavaScript, feature non-standard semantics of operators (e.g. greedy/lazy Kleene star), as well as additional features such as capturing groups and references. While symbolic execution of programs containing RegExes appeals to string solvers natively supporting important features of RegEx, such a string solver is hitherto missing. In this paper, we propose the first string theory and string solver that natively provide such a support. The key idea of our string solver is to introduce a new automata model, called prioritized streaming string transducers (PSST), to formalize the semantics of RegEx-dependent string functions. PSSTs combine priorities, which have previously been introduced in prioritized finite-state automata to capture greedy/lazy semantics, with string variables as in streaming string transducers to model capturing groups. We validate the consistency of the formal semantics with the actual JavaScript semantics by extensive experiments. Furthermore, to solve the string constraints, we show that PSSTs enjoy nice closure and algorithmic properties, in particular, the regularity-preserving property (i.e., pre-images of regular constraints under PSSTs are regular), and introduce a sound sequent calculus that exploits these properties and performs propagation of regular constraints by means of taking post-images or pre-images. Although the satisfiability of the string constraint language is undecidable, we show that our approach is complete for the so-called straight-line fragment. We evaluate the performance of our string solver on over 195000 string constraints generated from an open-source RegEx library. The experimental results show the efficacy of our approach, drastically improving the existing methods in both precision and efficiency.

==> motivating-example-new.tex <==
%!TEX root = main.tex

\section{Motivating Examples}\label{sec:mot}

We illustrate our method 
\subsection{Worked Out Example \#1}
\begin{figure}[tb]
\begin{center}
\begin{minted}[linenos]{javascript}
function normalize(decimal) {
  const decimalReg = /^(\d+)\.?(\d*)$/;
  var   decomp     = decimal.match(decimalReg);
  var   result     = "";
  if (decomp) {
    var integer    = decomp[1].replace(/^0+/, "");
    var fractional = decomp[2].replace(/0+$/, "");
    if (integer    !== "") result = integer; else result = "0"; 
    if (fractional !== "") result = result + "." + fractional;
  }
  return result;
}
\end{minted}
\end{center}

\caption{Normalize a decimal by removing the leading and trailing zeros}
\label{fig-run-exmp}

\end{figure}

We use the JavaScript program in Fig.~\ref{fig-run-exmp} as a th example to
illustrate our approach. %The example been adapted from typical JavaScript
%applications.
 The function {\tt normalize}   removes leading and trailing zeros from a decimal string with the input %a string variable 
{\tt decimal}. For instance, 
%we get results
 \texttt{normalize("0.250") == "0.25"},
 \texttt{normalize("02.50") == "2.5"},
 \texttt{normalize("025.0") == "25"},
and finally  \texttt{normalize("0250") == "250"}.

%\tl{should the "and" in dblp be removed? Alice Brown, John Smith}\zhilin{I am referring to the bibtex style. Both ACM and DBLP bibtex style contain ``and''}

In the function body, the input {\tt decimal} %of the function {\tt normalize} 
is matched to a regular expression {\tt decimalReg}\,=\,{\tt /\^{}({\footnotesize\textbackslash}d+){\footnotesize\textbackslash}.?({\footnotesize\textbackslash}d*)\$/}, which requires that  the input comprises a digit sequence representing the integer part of the input, possibly followed by a dot symbol (the decimal point) as well as another digit sequence representing the fractional part. The anchors  \verb!^! and \verb!$! denote the beginning and the end of the input, respectively. Note that  {\tt decimalReg} utilizes two capturing groups, namely, {\tt ({\footnotesize\textbackslash}d+)} and {\tt ({\footnotesize\textbackslash}d*)}, to record the integer and fractional part of the decimal. The expression {\tt {\footnotesize\textbackslash}.?} specifies that the dot symbol is optional, namely, it may not occur in the input. Moreover,  the regular expression utilizes the \emph{greedy} semantics of the quantifier {\tt +} to enforce that {\tt {\footnotesize\textbackslash}d+} is matched by the whole string if the input does not contain any dots. For instance, if ${\tt decimal} = \texttt{"0250"}$, then {\tt ({\footnotesize\textbackslash}d+)} is matched by \texttt{"0250"} and  {\tt ({\footnotesize\textbackslash}d*)} is matched by the empty string. 
%\tl{i guess here we want to express that the greedy semantics is crucial; the standard nondeterministic semantics does not meet our requirement?}
%Nevertheless, 
Note that the greedy semantics is crucial here, because with standard \emph{non-deterministic} semantics the {\tt ({\footnotesize\textbackslash}d+)} could also (incorrectly) by matched by \texttt{"02"}, and {\tt ({\footnotesize\textbackslash}d*)} by \texttt{"50"}.

  The result of the matching, which is an array of strings, is stored in the variable {\tt decomp}. 
%Since there are two capturing groups in {\tt decimalReg}, the array {\tt format} is of length 3.
%
Then the leading zeros are trimmed by applying {\tt replace(/\^{}0+/, "")} to {\tt decomp[1]} and the result is stored in the variable {\tt integer}. Similarly, the trailing zeros are trimmed by {\tt replace(/{}0+\$/, "")} to {\tt decomp[2]} and the result is stored in {\tt fractional}. The greedy semantics of {\tt 0+} is used to trim \emph{all} the leading/trailing zeros.
%
If {\tt integer} is empty, the return value gets a default value \texttt{"0"}. If {\tt fractional} is empty, then the return value is {\tt integer}. Otherwise, the return value joins {\tt integer} and {\tt fractional} with the dot symbol. 

A natural post-condition of {\tt normalize} is that the result
contains neither leading nor trailing zeros. This post-condition has
to be established by the function on \emph{every} execution path.  As
an example, consider the path shown in Fig.~\ref{fig-run-exmp-path},
in which the branches taken in the program are represented as
\texttt{assume} statements. The negated post-condition is captured by
the regular expression in the last \texttt{assume}. For this path, the
post-condition can be proved by showing that the program in
Fig.~\ref{fig-run-exmp-path} is infeasible: there does not exist an
initial value {\tt decimal} so that no assumption fails and the
program executes to the end.
\begin{figure}[tb]
\begin{center}
\begin{minted}[linenos]{javascript}
  const decimalReg = /^(\d+)\.?(\d*)$/;
  var decomp = decimal.match(decimalReg);
  var result = "";
  assume (decomp!==null);
  var integer = decomp[1].replace(/^0+/, "");
  var fractional  = decomp[2].replace(/0+$/, "");
  assume (integer !== ""); 
  result1 = integer;
  assume (fractional !== ""); 
  result2 = result1 + "." + fractional;
  assume (/^0\d+.*|.*\.\d*0$/.test(result2));
\end{minted}
\end{center}
\label{fig-run-exmp-path}

\caption{Symbolic execution of a path of the JavaScript program in Fig.~\ref{fig-run-exmp}}

\end{figure}

To enable symbolic execution of the JavaScript programs like in Fig.~\ref{fig-run-exmp}, we need to model the greedy semantics of {\tt +} and the matching of capturing groups. To this end, we propose the use of \emph{prioritized streaming string transducers} (PSST, Section~\ref{sect:psst}). The extraction of {\tt decomp[1]} from {\tt decimal}, namely {\tt decimal}. {\tt match(decimalReg)[1]}, can be modeled by a PSST $\cT_{\tt extract_{decimalReg,1}}$, where the priorities are used to capture the greedy semantics of $+$ (see Definition~\ref{def-regex-semantics} in Section~\ref{sec-rwre}) and the string variables are used to record the matches of capturing groups. %Similarly for  
The extraction of {\tt decomp[2]} can be handled in a similar way. Moreover, the functions {\tt replace(/\^{}0+/, "")} and {\tt replace(/0+\$/, "")}  can also be modeled by PSSTs $\cT_{\scriptsize\tt replace(\mbox{\tt /\^{}0+/, ""})}$ and $\cT_{\scriptsize\tt replace(\mbox{\tt /0+\$/, ""})}$.

After some further simplifications, we arrive at the following program
in our string-manipulating language, capturing Fig.~\ref{fig-run-exmp-path}.  In
the program, $\Aut_{\scriptsize\mbox{\tt/.+/}}$, $\Aut_{\tt decimalReg}$
and
$\Aut_{\scriptsize\mbox{\tt /\^{}0\textbackslash
    d+.*|.*{\scriptsize\textbackslash}.\textbackslash d*0\$/}}$ denote
finite-state automata corresponding to the regular expressions, and
the assumptions are encoded using \textsf{assert} (using the same
terminology as \cite{CHL+19}):
%
\begin{eqnarray}\label{eqn:exmp}
& & \ASSERT{\tt decimal \in \Aut_{decimalReg}};\nonumber \\
& & \sf integer  := \tt  \cT_{\tt replace(\mbox{\scriptsize \tt /\^{}0+/, ""})}(\cT_{\tt extract_{decimalReg,1}}(decimal));\nonumber \\
& & \sf fractional  := \tt  \cT_{\scriptsize\tt replace(\mbox{\tt /0+\$/, ""})}(\cT_{\tt extract_{decimalReg,2}}(decimal)); \\
&&  \ASSERT{\tt integer \in \Aut_{\scriptsize\mbox{\tt/.+/}}}; 
%&&  \tt result1 := integer;\nonumber\\
\ASSERT{\tt fractional \in \Aut_{\scriptsize\mbox{\tt/.+/}}}; \nonumber\\
 && \tt result2 := integer \concat ``." \concat fractional; \nonumber\\
 && \ASSERT{\tt result2 \in \Aut_{\scriptsize\mbox{\tt /\^{}0\textbackslash d+.*|.*{\scriptsize\textbackslash}.\textbackslash d*0\$/}}}; \nonumber
\end{eqnarray}


At first, we show that the pre-images of regular languages under PSSTs are regular (see Lemma~\ref{lem:psst_preimage}).
Then, path feasibility of the program in \eqref{eqn:exmp} can be checked by following the ``backward'' reasoning approach from \cite{CHL+19}.
First, we compute the pre-images of regular languages under the concatenation operation and remove the last assignment statement. Then, we compute the pre-images of regular languages under the PSSTs $\cT_{\tt extract_{decimalReg,2}}$ as well as $\cT_{\scriptsize\tt replace(\mbox{\tt /0+\$/, ""})}$, and remove the second assignment statement. Similarly for the first assignment statement. In the end, a program containing only regular membership queries (but possibly including disjunctions) is obtained, whose feasibility is reduced to checking the nonemptiness of the intersection of regular languages, which is known to be decidable (\pspace-complete). (See Appendix~\ref{app-br-mot-exmp} for more details.)

\input{example2}


==> prel.tex <==
%!TEX root = main.tex

\section{Preliminaries}\label{sec:prel}

Throughout the paper, $\Int^+$ denotes the set of positive integers, and  $\nat$ denotes the set of natural numbers. Furthermore, for $n\in \Int^+$, let $[n]:=\{1, \ldots, n\}$. 

We use $\Sigma$ to denote a finite set of letters, called \emph{alphabet}. Moreover, we use $\nullchar$ to denote a special null symbol and assume that  $\nullchar \not \in \Sigma$. 
A \emph{string} over $\Sigma$ is a finite sequence of letters from $\Sigma$. We use $\Sigma^*$ to denote the set of strings over $\Sigma$ and $\varepsilon$ to denote the empty string. Moreover, for convenience, we use $\Sigma^\varepsilon$ to denote $\Sigma \cup \{\varepsilon\}$. A string $w'$ is called a \emph{prefix} of $w$ if $w = w'w''$ for some string $w''$. We use $\pref(w)$ to denote the set of prefixes of $w$. For a prefix $w_1$ of $w$, let $w = w_1 w_2$, then we use $w_1^{-1}w$ to denote $w_2$.

\begin{definition}[Finite-state automata] \label{def:nfa}
	A \emph{(nondeterministic) finite-state automaton}
	(\FA{}) over a finite alphabet $\ialphabet$ is a tuple $\Aut =
	(\ialphabet, \controls, q_0, \finals, \transrel)$ where 
	$\controls$ is a finite set of 
	states, $q_0\in \controls$ is
	the initial state, $\finals\subseteq \controls$ is a set of final states, and 
	$\transrel\subseteq \controls \times 
	\ialphabet^\varepsilon \times  \controls$ is the
	transition relation. 
\end{definition}

For an input string $w$, a \emph{run} of $\Aut$ on $w$
%(with $a_0 = \EndLeft$ and $a_{n+1} = \EndRight$)
is a sequence $q_0 \sigma_1 q_1 \ldots \sigma_n q_n$ such that $w = \sigma_1 \cdots \sigma_n$ and $(q_{j-1}, \sigma_{j}, q_{j}) \in
\transrel$ for every $j \in [n]$.
The run is said to be \defn{accepting} if $q_n \in \finals$.
A string $w$ is \defn{accepted} by $\Aut$ if there is an accepting run of
$\Aut$ on $w$. In particular, the empty string $\varepsilon$ is accepted by $\Aut$ if $q_0 \in F$. The set of strings accepted by $\Aut$, i.e., the language \defn{recognized} by $\Aut$, is denoted by $\Lang(\Aut)$.
%Since we deal with computational complexity in the sequel, we define
The \defn{size} $|\Aut|$ of $\Aut$ is defined as the cardinality of the set $Q$ of states, which will be 
used when the computational complexity is concerned.

For convenience, for $a \in \Sigma$, we use $\delta^{(a)}$ to denote the  relation $\{(q, q') \mid (q, a, q') \in \delta\}$.
